Measurement of the Branching Fraction of $\Lambda_c^+ \to p K_S^0 \pi^0$ at Belle

We report a precise measurement of the ratio of branching fractions $\mathcal{B}(\Lambda_c^+\to p K_S^0 \pi^0)/\mathcal{B}(\Lambda_c^+\to p K^- \pi^+)$ using 980 fb$^{-1}$ of $e^+e^-$ data from the Belle experiment. We obtain a value of $\mathcal{B}(\Lambda_c^+\to p K_S^0 \pi^0)/\mathcal{B}(\Lambda_c^+\to p K^- \pi^+)=0.339\pm 0.002\pm 0.009$, where the first and second uncertainties are statistical and systematic, respectively. This Belle result is consistent with the previous measurement from the CLEO experiment but has a fivefold improvement in precision. By combining our result with the world average $\mathcal{B}(\Lambda_c^+\to p K^- \pi^+)$, we obtain the absolute branching fraction $\mathcal{B}(\Lambda_c^+\to p K_S^0 \pi^0)=(2.12\pm 0.01\pm 0.05 \pm 0.10)\%$, where the uncertainties are statistical, systematic, and the uncertainty in the absolute branching fraction scale $\mathcal{B}(\Lambda_c^+\to p K^- \pi^+)$, respectively. This measurement can shed light on hadronic decay mechanisms in charmed baryon decays.

==> acknowledgements.tex <==
% Please paste this acknowledgement into your latex file.
%
% 2022.11.09 updated after IB/spokespersons proposal and vote
% 2019.10.06 updated Russia
% 2019.08.25 updated Korea (third attempt), rephrased multi-grant numbering
% 2019.08.12 updated Korea (second attempt)
% 2019.98.08 updated Korea
% 2019.02.01 updated Austria
% 2018.10.23 updated Russia (short only)
% 2018.10.16 updated Spain
% 2018.07.19 updated computing/network, Russia, Australia, Korea, Fudan 
% 2018.01.31 updated Spain 
% 2018.01.08 all acronyms defined as asked from 
% 2017.12.14 updated China, fixed Korea formatting
% 2017.08.31 updated Korea
% 2017.05.25 updated Spain
% 2017.03.17 updated Korea, Czechia
% 2017.01.26 updated SINET5 (short only) 
% 2016.10.15 added China new No., removed MEXT+JSPS (Iijima-san),
% 	     Austria, updated SINET5 and Korean (Long only) 
% 2015.12.17 added China new No., Germany EXC, Taiwan, Spain
% 2015.08.25 updated Korea
% 2015.08.11 removed Australian Department of Industry, Innovation, 
%                    Science and Research (long); DIISR (short)
% 2015.04.27 add CCEPP (China)
% 2014.11.14 spelled out Korea & Spain FA (APS request, Long only)
% 2014.09.30 updated China grant #s (Long only)
% 2014.09.01 delete WCU (both). added three contract No.'s and 
%            delete one contract No.'s in long version
% 2014.07.28 added grant No. P 26794-N20 for Austria
% 2014.03.31 corrected "WCU program of the Ministry <of> Education"
% 2014.02.25 updated Czech contract no. (Long only)
% updated  2014.01.29 added Center for Korean J-PARC Users (Long only)
% updated  2013.11.20 included mods done by APS editor (Long only)
% updated  2013.09.19 new Korean part
% updated  2013.07.31 added two contract No.'s for China (Long only)
%
%***** Acknowledgments *****

%----------- Long version, for most papers ----------- 
This work, based on data collected using the Belle detector, which was
operated until June 2010, was supported by 
the Ministry of Education, Culture, Sports, Science, and
Technology (MEXT) of Japan, the Japan Society for the 
Promotion of Science (JSPS), and the Tau-Lepton Physics 
Research Center of Nagoya University; 
the Australian Research Council including grants
DP210101900, % Urquijo
DP210102831, % Sevior
DE220100462, % Hsu
LE210100098, % Infrastructure
LE230100085; % Infrastructure
Austrian Federal Ministry of Education, Science and Research (FWF) and
FWF Austrian Science Fund No.~P~31361-N36;
National Key R\&D Program of China under Contract No.~2022YFA1601903,
National Natural Science Foundation of China and research grants
No.~11575017,
No.~11761141009, 
No.~11705209, 
No.~11975076, 
No.~12135005, 
No.~12150004, 
No.~12161141008, 
and
No.~12175041, 
and Shandong Provincial Natural Science Foundation Project ZR2022JQ02;
the Czech Science Foundation Grant No. 22-18469S;
Horizon 2020 ERC Advanced Grant No.~884719 and ERC Starting Grant No.~947006 ``InterLeptons'' (European Union);
the Carl Zeiss Foundation, the Deutsche Forschungsgemeinschaft, the
Excellence Cluster Universe, and the VolkswagenStiftung;
the Department of Atomic Energy (Project Identification No. RTI 4002), the Department of Science and Technology of India,
and the UPES (India) SEED finding programs Nos. UPES/R\&D-SEED-INFRA/17052023/01 and UPES/R\&D-SOE/20062022/06; 
the Istituto Nazionale di Fisica Nucleare of Italy; 
National Research Foundation (NRF) of Korea Grant
Nos.~2016R1\-D1A1B\-02012900, 2018R1\-A2B\-3003643,
2018R1\-A6A1A\-06024970, RS\-2022\-00197659,
2019R1\-I1A3A\-01058933, 2021R1\-A6A1A\-03043957,
2021R1\-F1A\-1060423, 2021R1\-F1A\-1064008, 2022R1\-A2C\-1003993;
Radiation Science Research Institute, Foreign Large-size Research Facility Application Supporting project, the Global Science Experimental Data Hub Center of the Korea Institute of Science and Technology Information and KREONET/GLORIAD;
the Polish Ministry of Science and Higher Education and 
the National Science Center;
the Ministry of Science and Higher Education of the Russian Federation
and the HSE University Basic Research Program, Moscow; % from 15.04.2021
University of Tabuk research grants
S-1440-0321, S-0256-1438, and S-0280-1439 (Saudi Arabia);
the Slovenian Research Agency Grant Nos. J1-9124 and P1-0135;
Ikerbasque, Basque Foundation for Science, and the State Agency for Research
of the Spanish Ministry of Science and Innovation through Grant No. PID2022-136510NB-C33 (Spain);
the Swiss National Science Foundation; 
the Ministry of Education and the National Science and Technology Council of Taiwan;
and the United States Department of Energy and the National Science Foundation.
These acknowledgements are not to be interpreted as an endorsement of any
statement made by any of our institutes, funding agencies, governments, or
their representatives.
We thank the KEKB group for the excellent operation of the
accelerator; the KEK cryogenics group for the efficient
operation of the solenoid; and the KEK computer group and the Pacific Northwest National
Laboratory (PNNL) Environmental Molecular Sciences Laboratory (EMSL)
computing group for strong computing support; and the National
Institute of Informatics, and Science Information NETwork 6 (SINET6) for
valuable network support.
S. B. Yang and J. K. Ahn acknowledge the support provided by NRF Grant No. 2018R1A6A3A01012138, No. 2018R1A5A1025563, No. 2019K1A3A7A09034960, and No. 2021R1C1C2012925 and by the POSCO Science Fellowship of POSCO TJ Park Foundation.
